Seiberg-Witten Floer Spectra and Contact Structures

In this article, the author defines an invariant of rational homology 3-spheres equipped with a contact structure as an element of a cohomotopy set of the Seiberg-Witten Floer spectrum as defined in Manolescu (2003). Furthermore, in light of the equivalence established in Lidman & Manolescu (2018a) between the Borel equivariant homology of said spectrum and the Seiberg-Witten Floer homology of Kronheimer & Mrowka (2007), the author shall show that this homotopy theoretic invariant recovers the already well known contact element in the Seiberg-Witten Floer cohomology (vid. e.g. Kronheimer, Mrowka, Ozsv\'ath & Szab\'o 2007) in a natural fashion. Next, the behaviour of the cohomotopy invariant is considered in the presence of a finite covering. This setting naturally asks for the use of Borel cohomology equivariant with respect to the group of deck transformations. Hence, a new equivariant contact invariant is defined and its properties studied. The invariant is then computed in one concrete example, wherein the author demonstrates that it opens the possibility of considering scenarios hitherto inaccessible.

==> Makefile <==
.POSIX:
.SUFFIXES:

FIG = figs/left_trefoil_ps \
      figs/legendrian_left_trefoil_tb_minus_7_rot_0_ps \
	figs/minus_eight_left_trefoil_ps \
	figs/minus_eight_left_trefoil_blown_up_ps \
	figs/minus_eight_left_trefoil_blown_up_simplified_ps \
	figs/minus_eight_left_trefoil_ready_for_cover_ps \
	figs/minus_eight_left_trefoil_untied_ps \
	figs/left_trefoil_ready_for_branched_cover_ps \
	figs/left_trefoil_double_branched_cover_ps \
	figs/minus_eight_left_trefoil_double_cover_ps \
	figs/minus_eight_left_trefoil_spin_ps \
	figs/minus_eight_left_trefoil_blown_up_spin_ps \
	figs/left_trefoil_ready_for_branched_cover_spin_ps \
	figs/left_trefoil_double_branched_cover_spin_ps \
	figs/minus_eight_left_trefoil_ready_for_cover_spin_ps \
	figs/minus_eight_left_trefoil_double_cover_spin_ps \
	figs/lens_12_7_step_1_ps \
	figs/lens_12_7_step_2_ps \
	figs/lens_12_7_step_3_ps \
	figs/lens_12_7_step_4_ps \
	figs/lens_12_7_step_5_ps \
	figs/lens_12_7_final_ps \
	figs/lens_12_7_contact_1_ps \
	figs/lens_12_7_contact_2_ps \
	figs/lens_12_7_contact_3_ps

SRC = main article notation maths bib intro sw review \
      contact recovery cover borel d3 spinc \
      uniq

OBJ = main.log main.aux main.ps main.pdf main.dvi

.PHONY: all
all: main.pdf

main.pdf: main.ps
	gs -dBATCH -dNOPAUSE -sDEVICE=pdfwrite -sOutputFile=$@ $<
main.ps: main.dvi
	dvips -q $<
main.dvi: $(SRC:=.tex) $(FIG:=.tex)
	tex -interaction nonstopmode \
		-halt-on-error \
		-file-line-error \
		main.tex
	rm -fv main.log

.PHONY: clean
clean:
	rm -fv $(OBJ) 


==> figs/minus_eight_left_trefoil_blown_up_simplified_ps.tex <==
\vbox{%
	\baselineskip = 0pt%
	\hbox{\hskip105bp}%
	\vbox{\vskip67.5bp}%
	\vtop{\vskip67.5bp}%
	\special{psfile=figs/minus_eight_left_trefoil_blown_up_simplified.ps}%
}%

